Semantics-aware Dataset Discovery from Data Lakes with Contextualized Column-based Representation Learning

Dataset discovery from data lakes is essential in many real application scenarios. In this paper, we propose Starmie, an end-to-end framework for dataset discovery from data lakes (with table union search as the main use case). Our proposed framework features a contrastive learning method to train column encoders from pre-trained language models in a fully unsupervised manner. The column encoder of Starmie captures the rich contextual semantic information within tables by leveraging a contrastive multi-column pre-training strategy. We utilize the cosine similarity between column embedding vectors as the column unionability score and propose a filter-and-verification framework that allows exploring a variety of design choices to compute the unionability score between two tables accordingly. Empirical evaluation results on real table benchmark datasets show that Starmie outperforms the best-known solutions in the effectiveness of table union search by 6.8 in MAP and recall. Moreover, Starmie is the first to employ the HNSW (Hierarchical Navigable Small World) index for accelerate query processing of table union search which provides a 3,000X performance gain over the linear scan baseline and a 400X performance gain over an LSH index (the state-of-the-art solution for data lake indexing).

==> src/cover.tex <==
\newcommand{\reminder}[1]{{\mbox{$<==$}} [[[ { \bf #1 } ]]] {\mbox{$==>$}}}
\newcommand{\response}{\smallskip\noindent\textbf{\textcolor{blue}{Response: }}}

\begin{center}
	\huge\textbf{Response to Reviewer Comments}\\
\end{center}

% \skip

\noindent We thank the reviewers for their thoughtful reviews and constructive comments. 
The paper has gone through a thorough revision process. 
We believe that the new version has comprehensively addressed all comments/suggestions mentioned in the reviews. 

% \renee{change hard-coded number to references to sections/figures}\grace{Done except for conclusion}
% \begin{itemize}
%     \item Presentation:  A number of the comments were on presentation specifically asking for more discussion of the motivation for the design choices, including the decision to use the "hammer" of deep learning.  To address this, we have done major re-writes in the introduction to better describe the state-of-the-art which indeed uses the light-weight (embedding/ontologic) solutions that the reviewers mention and how our deep learning approach is more than a minor improvement in accuracy over these.  We have also rewritten Section~\ref{sec:offline} as suggested by R4 to include an algorithm and more detailed discussion/motivation of design choices.  And we have replaced conclusion with a future work section that stresses the promise of our innovations in not just unionable table search, but in other forms of table discovery and understanding.
%     \item  Experiments:  We have added a microbenchmark as requested to evaluate the effect of  randomly picking tables as negative examples.  We show that even as the assumption (likelihood) that random tables are not unionable decreases that this has a negligible effect on the accuracy of our approach.  To motivate the inclusion of context, we further highlight it in the introduction as well as the running example in Figure~\ref{fig:motivation}.  And to evaluate its importance we have added  the baseline method \emph{SingleCol} (Section~\ref{subsubsec:baselines} which is a version of our approach without context information), to all experiments in Figure~\ref{fig:error_santos}.  This quantifies the performance loss when removing the contextual information.
% \end{itemize}

\section*{Response to  Comments by Meta-Reviewer}

{\it \noindent {\bf Meta Reviewer}: 
	The paper is descriptive rather than prescriptive. (R4's W1 and D1, R5's W1). The reviewers would like to see the random sampling for counterexamples trick emphasized more (R4's D3), and discussed in greater depth, maybe hammered home with a probabilistic argument or experiments that the effect of picking randomly has a negligible effect on the loss function for a sufficiently large batch size (R4's D2 and R6's O2). The reviewers would like to see more discussion of the motivation for the choice of models --- was there a specific methodology used to choose them?
	
	- The reviewers would like to see some justification for deploying the deep learning hammer as opposed to some lighter-weight solutions that may not be quite as effective, but give the reader a much deeper understanding of the problem being solved (R4's W2 and R6's O1).
	
	There needs to be a discussion of future work (R5 W3)
	
	While we urge the authors to take into account all of the comments, there are a number that the reviewers feel really must be resolved before the paper can be accepted. These include R4's W3, D5, D7, and D8.
	
}

%\renee{I think this either needs to be more detailed and point-by-point or removed.}\jin{I move the summary made by you to the response to meta-reviewer.}
\response  Thank you for your constructive comments, we have prepared a comprehensive revision to address these items.
We summarize the major changes below and then respond to each itemized review comment made by the reviewers.
We made the following changes to address the comments on Presentation:
\begin{itemize}
    \item A number of the comments ask for more discussion of the motivation for the design choices, including the decision to use the "hammer" of deep learning.  To address this, we have done major re-writes in the introduction to better describe the state-of-the-art which indeed uses the light-weight (embedding/ontologic) solutions that the reviewers mention and how our deep learning approach is more than a minor improvement  over these.  
    \item We have rewritten Section~\ref{sec:offline} as suggested by R4 to include an algorithm and more detailed discussion/motivation of design choices.  
    \item We have extended the conclusion section with a discussion of future work that stresses the promise of our innovations in not just unionable table search, but in other forms of table discovery and understanding.
\end{itemize}

We made the following changes in the Experiments:
\begin{itemize}
    \item  We have added a microbenchmark as requested to evaluate the effect of  randomly picking tables as negative examples.  We show that even as the assumption (likelihood) that random tables are not unionable decreases that this has a negligible effect on the accuracy of our approach.  
    \item To motivate the inclusion of context, we further highlight it in the introduction as well as the running example in Figure~\ref{fig:motivation}.  And to evaluate its importance we have added  the baseline method \emph{SingleCol} (Section~\ref{subsubsec:baselines} recall that \emph{SingleCol} is a version of our approach without context information), to all experiments in Figure~\ref{fig:error_santos}.  This quantifies the performance loss when removing the contextual information.
\end{itemize}

%%%%%%%%%%%%
\iffalse
The revisions we have made can be summarized as following:
\begin{itemize}
	\item We provide more background information to clarify the problem setting as well as our contributions.
	\item We add additional experiments to justify our methodology and design choices, such as the one mentioned in R4D1 and R4D2.
	\item We polish our presentation and add the discussion about future work.
\end{itemize}
\fi

For more details, please refer to answers to each reviewer's comments in the following.

\section*{Response to Comments by  Reviewers}

\subsection*{Responses to Reviewer \#4}

{\it \noindent {\bf R4W1}: The paper leans heavily into machine learning techniques as a solution to the multi-column matching problem, but much of the focus is just on describing the model in its final iteration. I would expect to see a greater focus on the design principles behind the model, testing of assumptions, and/or an in-depth study of the final model parameters... something to help the reader understand the generalizability of the approach beyond the experimental data. (D1, D2, D4, D7, D8)
}

\response We have thoroughly addressed this point and details are provided in each of the D comments below.
%We provide more technical details and experimental results about the issues you mentioned here.
%Please refer to the answers  in each D below for more details. 
\smallskip

{\it \noindent {\bf R4W2}: On a related note, machine learning is a very heavyweight solution. Is it possible that lighter-weight heuristics could achieve a comparable end? For example, would a solution that computes the information content of a column's summary (i.e., token set, column embedding, etc...), be able to achieve a similar end by ``downweighting'' column pairs in the bipartite matching that appear frequently in the data lake. (D1)
}\\
{\it \noindent {\bf R4D1}: It would be useful to have a bit more insight into why the model works the way it does. For example, what is the context-embedding trick recording? Is it picking up on the fact that some classes of attribute (e.g., dates) are less informative and down-weighting their similarity, or is it actually embedding some form of ``context'' into the date (``2012 associated with California and Robin''). If so, what kind of context?
}

\response  Light-weight heuristics such as those mentioned by the reviewer are indeed the state-of-the-art and are described in the related work (Section~\ref{sec:related}).  We agree with the reviewer however that they need to be described in the introduction in order to justify the use of our more heavy-weight machine learning approach.  
%We want to clarify that the ``light-weighted'' solutions that computes the information content of a column's summary has been proposed in the previous study [39]. 
The use of column summaries was explored as early as 2009~\cite{DBLP:journals/pvldb/CafarellaHK09,DBLP:conf/sigmod/YakoutGCC12} and more recently using column embeddings (including word embeddings) and ontology mappings~\cite{DBLP:journals/pvldb/NargesianZPM18}.  
Note that this last approach does include a mechanism for modeling context in a way that is similar in motivation (but more mathematically sophisticated) to what the review suggests regarding down-weighting.  
Specifically their {\em ensemble unionability} picks the signal (column unionability score) that is the most surprising (unlikely) within the context of all column unionability scores in a data lake -- modeling a form of data lake context.  Their approach~\cite{DBLP:journals/pvldb/NargesianZPM18} was later augmented with regular expressions over columns ($D^3L$~\cite{DBLP:conf/icde/BogatuFP020}) and with relationship embeddings (SANTOS~\cite{santos23}).  The latter two approaches showed improvements over~\cite{DBLP:journals/pvldb/NargesianZPM18} (as they incorporate more signals), and hence we compare directly against $D^3L$ and SANTOS.  
We have added this discussion to the introduction.  
%However, the experimental results in the previous studies shows that the performance of [39] is consistently worse than $D^3$L [2] and SANTOS [22].
%Thus in the experiments of this paper, we only compare with [2] and [22].
%We add such clarification in Section 5.1.4 of the revised version.

For the motivation of including ``context'', we further highlight it in the introduction as well as the running example in Figure~\ref{fig:motivation}.  
We have also clarified that while previous approaches have used the context of the data lake to in some sense differentiate the weight or importance of different attribute pairs, our context mechanism is embedding the tuple context, e.g., (``2012 associated with California and Robin''). 
We have also stressed that the baseline method \emph{SingleCol} mentioned in Section~\ref{subsubsec:baselines} is a version without context information, we add more experimental results in Figure~\ref{fig:error_santos} to show that there is a performance loss if  contextual information is removed.

\smallskip

{\it \noindent {\bf R4W3}: Why were experiments run on only a small sample of query tables from the TUS benchmarks? 100-150 datasets is not a very large data lake; If this is a scalability issue, that should be discussed.
}

\response No, this is not a scalability issue.  
In addition to the effectiveness experiment, we also evaluated scalability of Starmie on large data lakes with up to 50M tables (see Section~\ref{subsec-scal} and Figure~\ref{fig:scal}). For the effectiveness experiments (Section~\ref{subsec-eff}), we used the \emph{labeled} datasets to have a fair comparison with SANTOS~\cite{santos23} (as this is the sample that they used and for which they provided ground truth).  
While TUS~\cite{DBLP:journals/pvldb/NargesianZPM18} provides ground truth for their full benchmark, TUS considers tables unionable based  on column semantics. 
SANTOS~\cite{santos23} considers tables unionable if both their columns and relationship semantics match.  They provide ground truth for only this small sample of the TUS benchmark.

We highlight this difference in Section~\ref{subsubsec:datasets} to ensure this point is clear as we agree with the reviewer that it is important.


% We want to clarify that actually in the experiments of effectiveness (Section~\ref{subsec-eff}) and efficiency (Section~\ref{subsec-scal}), we use different datasets.
% To evaluate the effectiveness, we need benchmarking datasets with \emph{ground truth} that are manually labeled. %Due to the limitation of human resources for creating such ground truth, the carnality of datasets for evaluating effectiveness is not so large, which is also similar in previous studies [2,22,39].

% Nevertheless, for the experiments of evaluating efficiency, we use much larger datasets including the WDC dataset that has 50 million tables.

\smallskip


{\it \noindent {\bf R4D2}: The paper's approach to unsupervised training of the model makes a key assumption that the probability of randomly drawing two tables that are unionable is negligible. It would be useful to quantify the impact of this assumption. e.g., this point could be addressed with a microbenchmark that relates the number of classes of table to the model's precision/recall, possibly with different levels of skew. (I do recognize that if a particular entity appears frequently enough in a data lake, unionability search is not quite as critical)
}

\response Thank you for your constructive comment. 
We add micro benchmarking experiments over the TUS Small benchmark in Section~\ref{subsubsec:micro} of the revised version.
It shows that the performance is not significantly influenced as the number of classes decreases (and hence the likelihood that random tables are not unionable also decreases).  
%Thus the assumption of our unsupervised training step should be fine.
\smallskip

{\it \noindent {\bf R4D3}: The core idea of the paper: Two randomly sampled data tables are unlikely to be examples of the same data is buried in Section 3.1. This is a very easy intuition to convey, and it should come across in the introduction when introducing the idea that the approach is self-supervised.
}

\response %Actually the point you mentioned here is a fundamental one that is applicable to all studies based on the contrastive learning paradigm.
We have added this to the introduction.
%rjm I think we don't want to emphasize this in the cover letter as the reviewer could then say "Oh the thing I thought was novel is not novel...
%This is indeed one of the general assumption made by contrastive learning algorithms like SimCLR.
We also clarify this assumption and add other relevant background related to contrastive learning in Section~\ref{subsec:bg} of the revised version.

{\it \noindent {\bf R4D4}: Section 3, and in particular Sections 3.1 and 3.2 are written in a very prescriptive style that makes them hard to follow. In general, I'm more interested in reading about why specific choices were made? For example, why was the specific set of augmentation operators in Table 1 chosen?	
}

\response We thank the reviewer for the suggestion and have rewritten Section~\ref{sec:offline} extensively.  Specifically, we added  justification on the design choices behind the augmentation operators Section~\ref{subsec:simclr} (for single-column) and Section~\ref{subsec:contextualized} (for multi-column).
Due to the large number of choices, we also conducted an ablation study to evaluate which one
performs the best for table discovery in Appendix B.  
This can also be found in our archive version~\cite{DBLP:journals/corr/abs-2210-01922}.  
We were unable to fit the full ablation study into the paper due to space, but we believe we have added the intuition to the paper as requested.  We found that the column sampling operator drop\_col performs the best and it is our main choice in our experiments.
% We are sorry for the ambiguity.
% We have added necessary background knowledge in Section 3.1 of the revised version for further clarification.

{\it \noindent {\bf R4D5}: In Section 3.2, the paper claims that the separator marker <s> for each column is somehow augmented with a summary of the column in the context of the table. This seems to rely on some property of the transformer that isn't clearly described. I *think* this is what Figure 6 is trying to get across, but I don't see it referenced anywhere in the prose.
}

\response We thank the reviewer for pointing this out. We have added clarification in the revised
Section~\ref{subsec:contextualized}. The special token <s> is used as the sequence start token in RoBERTa (as in the HuggingFace library) so we re-use the same token as column start token so that it is likely to capture the contextualized column representation.  
Our revision explains this and explains Figure~\ref{fig:match_nonmatch}.  

% Actually this issue is only in the implementation level instead of the property of the model. 
% It is based on the requirement of the tokenizer in the Hugging Face Transformer library, which is the most popular library for Transformers nowadays.
% We add the clarification of it in the revised version. 


{\it \noindent {\bf R4D6}:  In the first paragraph of Section 3.3, there's a quick mention that the tests also compare against row embeddings. This feels like a bit of an offhand remark, as it's not entirely clear to me why that would be a reasonable comparison. Is the idea that a row embedding somehow captures the idea of an "entity"?
	
 \noindent {\bf R4D7}: Different approaches for table augmentation are mentioned throughout Section 3, but the precise process used (and the design choices behind it) are never formalized -- The paper limits itself to a (very vague) summary sentence at the end of Section 3. I would like to know more about the exact process (and the reasoning behind it).
}

% \yuliang{TODO: mention that we took the suggestion of the reviewer}

\response % We are sorry for the ambiguity.
We thank the reviewer for the comment and we took your suggestion ({\em R3. Cut D6 if space is needed.}).
In the original version,
for ``compare against row embeddings'', we tried to describe 
the possible design choices for pre-processing.
We now leave the full discussion about these design choices (also for
the augmentation operators) to Appendix A and B.2 to avoid any confusion as you suggest.
In the main paper, we added a new Section \ref{subsec:pretbl} 
and Algorithm \ref{alg:pretable} to formally
describe our final choice of  operators: 
we use the average TF-IDF scores for cell scoring, the deterministic method for ordering, and rank all the rows by their average cell-level scores.
We also added more description in Section \ref{subsec:contextualized}
to motivate how we chose the data augmentation operators.
% % In the final version,  we use the average TF-IDF scores for cell scoring, the deterministic method for ordering and rank all the rows by their average cell-level scores.

% We clarify our presentation by 

% Actually in Section~\ref{subsec:contextualized} we just discuss some possible solutions for each step.

% To avoid ambiguity, we add a pseudo code (Algorithm~\ref{alg:pretable}) to describe the process in the revised version and move the full discussion to the appendix.
\smallskip

{\it \noindent {\bf R4D8}:  Figure 7 illustrates a scenario that I find very unlikely... one where every column in T is similar to virtually every column in S. This suggests that the scoring functions are not well normalized (which deserves further discussion), or that T and S contain a large number of identical columns. It would be useful to understand how often this happens in practice, as this may significantly simplify other parts of the algorithm. One way to quantify this would be to measure the CDF of the difference between LB and UB are for all pairs of distinct tables in a dataset. If this difference is nearly always zero, then the bipartite search is not adding a lot (otoh, in this scenario, one would also expect bipartite search to be nearly rarely, if ever, invoked, since the pruning heuristic would work just as well).
}

\response Quite right, Figure~\ref{fig:bp} is a ``made-up'' example to help readers better understand the algorithm rather than a case study from real datasets.  
We now clarify in the prose  that it is no way illustrative of real data distributions -- it is a deliberately chosen edge-case to help readers understand the algorithm. 
Unfortunately as the similarity score between pairs of tables cannot be normalized to a range, e.g. 0 to 1, it is not feasible to show a CDF of UB/LBs. 
Nevertheless, we illustrate the effectiveness of the lower and upper bounds in two alternative ways as (i) the query time of the pruning based approach equipped with LB/UB is less than that of the naive method without LB/UB, which is shown in Table~\ref{tab:metrics_runtime}; and (ii) we added the number of computations done for bipartite matching  with and without LB/UB pruning in Section~\ref{subsec-scal} in the revised version. 
Since the number of computations can be reduced with the help of the LB/UB, we feel the effectiveness of this approach on real is justified.
\smallskip

{\it \noindent {\bf R4 Minor Points}:  
M1. The acronym HNSW is used without definition on page 2.
M2. On page 2, a MAP score of 6.8 is given without context (is this good?)
M3. Consistency: At the end of Section 2.1, mathcal U is defined as a triple, but then used as a function.
M4. Addressing D3 might fix this, but the term "augmented" table feels a bit counterintuitive, given that the initial example of augmentation is sampling. "Perturbed" might be a better descriptor?
M5. Section 3.1, equation 1. Shouldn't the constraint in the denominator also include k $\neq$ j?
M6. The dotted line in Figure 7 does not print well. Suggest increasing the line weight	
}

\response We addressed all these presentation issues in the revised version.
Thank you for pointing them out.

\subsection*{Responses to Reviewer \#5}

{\it \noindent {\bf R5W1}: An in-depth discussion of experimental results is missing in several aspects. Instead of simply presenting the experimental results, a deep dive into the cause is essential.

The paper misses in depth cause analysis of experimental results. For instance, a detailed cases analysis of failed cases of Starmie is not presented in the paper. This may expose the weakness of the method and innovate future improvements. Also, why is R@k low for all methods for the TUS large dataset is not explained.
}

\response We have edited Section~\ref{sec:experiments} to add a deeper dive into causes including failure cases of Starmie.  We want to clarify that due to the limited availability of labeled ground truth, the highest value of R@k is restricted to different values on different datasets.
This setting is the same with previous studies [2,22,39].
We use a line named IDEAL in Figure~\ref{fig:p_r_all} to show this upper bound (which indeed is low as the reviewer points out).  For example, for SANTOS Small Benchmark and k=4, the number of correct answers is on average 13.  But with k=4 no algorithm can return all 13 correct answers (100\% recall), at best they can return 4 of the 13 (i.e., $\sim$30\% recall).  So this number is plotted in the IDEAL line.  Starmie achieves this IDEAL performance for small $k$ and comes close for larger $k$.
We added this clarification in Section~\ref{subsec-eff} of the revised version to make sure this is clear and that Starmie is achieving the ideal or close to ideal recall (and why the IDEAL is so low on TUS large).  
\smallskip

{\it \noindent {\bf R5W2}: There are several typos, grammar, formatting and layout issues in the paper. Please proofread and fix accordingly.

Here are a few presentation errors in the paper. Please note and fix.
* Algorithm 1 and Figure 3 may interchange position.
* Line 6 of Algorithm 1 is missing a "(".
* g in the last line of Algorithm 1 is not defined.
* On page 6, the second sentence in the first paragraph of section 4, "we first the table union ability scores..." is missing a verb.
}

\response We fixed these issues in the revised version. 
Thank you for pointing them out.
\smallskip

{\it \noindent {\bf R5W3}: Future direction of the paper is not mentioned in the paper.
	
A discussion of future direction may better influence future work in the area. For instance, how will the unsupervised method combine with existing supervised method? Will the framework be adaptable to table join search?
}

\response Thank you for your suggestion.
We add the discussion of future work in Section 7 of the revised version.  To make room for this, we reduced the old "summary" style conclusion.  

\subsection*{Responses to Reviewer \#6}

{\it \noindent {\bf R6O1}:  While I really enjoyed the thoroughness of the experiments, I felt like I was missing some simple baselines that used some simple heuristics to try to filter away semantically dissimilar tables. E.g. if there is a column with no good match in another table, mark those two tables as non-matching?
	
\noindent  {\bf R6O2}: As I explain in more detail below, I feel like the argument in the intro supporting the validity of the semantic mismatch problem could be made a lot stronger. How frequently does this failure mode happen? What is the impact when it does? You start to address this in 5.4 (which is great - more of this!!)
	
\noindent {\bf R6D1}:  Intro: do you have any sense as to the number of errors caused by not taking table semantics into account?
}

\response We hope the rewrites to the introduction that we did for R4W1/R4D1 clarifies that the baselines we use (including $D^3L$ and SANTOS) do use some simple heuristics like those you mention (and are the state-of-the-art).
For example, $D^3L$ uses Jaccard and simple attribute name matching among a few other heuristics to determine if columns are matching.  
SANTOS maps binary relationships to an ontology (YAGO) and uses this to determine if matching pair of columns should be considered matching.  
Actually it is very difficult to find a reasonable way to quantitatively illustrate how serious the semantic mismatch problem is in the dataset and how well each approach can solve it.  
We compare with the unsupervised baselines $D^3L$ and SANTOS, and with the supervised baselines SATO and Sherlock (both column matchers).  
And we proposed a baseline method \emph{SingleCol} mentioned in Section~\ref{subsubsec:baselines}.
Compared with the full version of \emph{Starmie}, \emph{SingleCol} does not use contextual information in the process of contrastive learning as described in Algorithm~\ref{alg:simclr}.  
Our goal was to tease out the influence of contrastive learning vs. context (note that context is also used in the supervised SATO).  
And the results in Figure~\ref{fig:error_santos} and Table~\ref{tab:map} show that \emph{Starmie} consistently outperforms \emph{SingleCol}, which illustrates the necessity of including contextual information in the process of contrastive learning.  
And the Starmie's outperformances of SATO which includes context in a similar way to Starmie shows the benefit of using contrastive learning over SATO's supervised approach.
\smallskip

{\it \noindent {\bf R6D2}: Wouldn't a naive solution be to pair tables that are "similar" and then find matching columns using existing methods? Or even having some min/max scoring where the min alignment can't be too low (i.e. avoid table C and table A unioning as in figure 1). I'm less familiar with the related work in this area but have people not done this already? Overall, I feel like the intro is missing a little grounding into that this table semantic mismatch is one of the major issues with table union search that is unaddressed by prior methods. You have a little of this in the paragraph of "While existing work has..." and Example 1.1, I think it could be a lot stronger. Add quantitative metrics if you can. Say you ran XX existing methods and found that X$\%$ of their errors involved this mismatch problem.
}

\response Quite right and yes, this naive solution was proposed in Octopus~\cite{DBLP:journals/pvldb/CafarellaHK09} for web tables (cluster tables then do simple schema matching), Table Union Search~\cite{DBLP:journals/pvldb/NargesianZPM18} showed a clear improvement over Octopus and then our baselines (SANTOS~\cite{santos23} and $D^3L$~\cite{DBLP:conf/icde/BogatuFP020}) improve on this. And yes, you are right that this background needs to be in the introduction.  
In response to comments from all reviewers we have provided better description of related work and the history of this area in the introduction.
Indeed the bipartite matching score for evaluating table unionablity in Section~\ref{subsec-setup} is borrowed from the previous study [39].
We do not aim at improving the table unionablity score in this paper.
Instead, our contribution lies in (i) we have more effective column representation approach compared with [39] as you mention; (ii) we explore more design choices like HNSW index and lower/upper bound to accelerate query processing of the overall framework.
We have revised the introduction and Section~\ref{subsec-setup} to more properly reflect our contributions.
\smallskip

{\it \noindent {\bf R6D3}: I was a bit confused as the loss function in 3.1 didn't have this notion of column alignment from 3.2 so I was a bit confused by how pairs of columns were aligned. I think what you do is actually treat each unit in 3.1 as a single column embedding and just embed them contextually. But algorithm 1 doesn't show columns/tables together, so I thought they were tables being embedding and contrasted.
}

\response We are sorry for the ambiguity.
We added more background information in Section~\ref{sec:offline} and made an extensive  revision to help reader better understanding the technical details.
Please refer to R4D4 to R4D7 for more details.
\smallskip

{\it \noindent {\bf R6D4}: In the experiments, you have the phrase "Figure 11 shows, for the same US congress members table, Jaccard similarity may retrieve an irrelevant table of dog competitions that also contains a similar “State” column, but the two tables are not semantically relevant.". When you say Jaccard similarity "may" retrieve...does it actually retriever or are you hypothesizing here?
}

\response We are sorry for the ambiguity.
It actually retrieves it and we are just describing our findings in the experiments.
We have fixed the wording in the revised version.
\smallskip

{\it \noindent {\bf R6D5}: Is the SingleCol baseline from 3.1 a contrastively trained one? How is it trained?
}

\response Yes, it is trained in the same way as Starmie.  
The only difference is that it does not include context.  
We have clarified this in the paper.  
Please refer to the response to R6O1.
